Comparing Multi-Index Stochastic Collocation and Multi-Fidelity Stochastic Radial Basis Functions for Forward Uncertainty Quantification of Ship Resistance

This paper presents a comparison of two multi-fidelity methods for the forward uncertainty quantification of a naval engineering problem. Specifically, we consider the problem of quantifying the uncertainty of the hydrodynamic resistance of a roll-on/roll-off passengers ferry advancing in calm water and subject to two operational uncertainties (ship speed and payload). The first four statistical moments (mean, variance, skewness, kurtosis), and the probability density function for such quantity of interest (QoI) are computed with two multi-fidelity methods, i.e., the Multi-Index Stochastic Collocation (MISC) method and an adaptive multi-fidelity Stochastic Radial Basis Functions (SRBF) algorithm. The QoI is evaluated via computational fluid dynamics simulations, which are performed with the in-house unsteady Reynolds-Averaged Navier-Stokes (RANS) multi-grid solver $\chi$navis. The different fidelities employed by both methods are obtained by stopping the RANS solver at different grid levels of the multi-grid cycle. The performance of both methods are presented and discussed: in a nutshell, the findings suggest that, at least for the current implementations of both algorithms, MISC could be preferred whenever a limited computational budget is available, whereas for a larger computational budget SRBFs seem to be preferable, thanks to its robustness to the numerical noise in the evaluations of the QoI.

==> _region_.tex <==
\message{ !name(misc.tex)}
\message{ !name(misc.tex) !offset(14) }
\begin{equation}\label{eq:CC_points}
t^{j}=\cos\left(\frac{(j-1) \pi}{K-1}\right), \quad 1\leq j \leq K,
\end{equation}
\message{ !name(misc.tex) !offset(-6) }


==> comparison_unified.tex <==
\begin{figure}[!t]
	\centering
	\subfigure[Expected value]{\includegraphics[width=1\textwidth]{Fig_MISC/comparison_mean_conv.png}}
	\subfigure[Standard deviation]{\includegraphics[width=1\textwidth]{Fig_MISC/comparison_std_conv.png}}
	\caption{Comparison of MISC and SRBF results: convergence of the expected value and standard deviation of $R_T$ versus computational cost. For the sake of readability, we plot the results for MISC starting with the 4th iteration. The first three iterations correspond to computational cost 1, 12, and 14, and give poor results.}
	\label{fig:EV_comparison}
\end{figure}

In this section the behavior of the two methods applied to the problem just described is illustrated.
To fairly compare the outcomes of the two UQ methodologies presented, no termination criteria are used for both methods, that are stopped when sufficient and comparable computational costs have been reached.

\begin{table}[!b]
\centering
\caption{Comparison of MISC and SRBF results: computational cost, expected value and standard deviation of $R_T$ for an intermediate iteration and at the final iteration.}\label{table:comparison}
\begin{tabular}{ccccc}
\toprule
\bf UQ method & \multicolumn{2}{c}{MISC} & \multicolumn{2}{c}{SRBF}\\
\midrule
Iteration                    & 14      & final   & 8       & final \\
Computational cost           & 900     & 4008    & 4638    & 4721 \\
$\mathbb{E}\left[R_T\right]$ & 52.0    & 53.3    & 51.7    & 52.2 \\
$\text{std}\left[R_T\right]$ & 26.9    & 22.4    & 21.4    & 21.0\\
\bottomrule
\end{tabular}
\end{table} 

\begin{figure}[!b]
	\centering
	\subfigure[MISC, iteration 14]{\includegraphics[width=0.45\textwidth]{Fig_MISC/pdf_iter13.png}}
	\subfigure[MISC, final iteration]{\includegraphics[width=0.45\textwidth]{Fig_MISC/pdf_iter30.png}}
	\subfigure[SRBF, iteration 8]{\includegraphics[width=0.45\textwidth]{Fig_RBF/Iter0033-Histogram.png}}
	\subfigure[SRBF, final iteration]{\includegraphics[width=0.45\textwidth]{Fig_RBF/Iter0053-Histogram.png}}
	\caption{Comparison of MISC and SRBF results: density function and histogram of (rescaled) frequencies of $R_T$. The histogram is computed using 25 bins for $n=10000$ samples of the response surface. The probability density function is estimated using the kernel smoothing estimate given by the Matlab's ksdensity function, enforcing positive support and with automatic selection of the bandwidth.
%the Matlab kernel smoothing function estimate given by \texttt{ksdensity} with positive support and automatic choice of the bandwidth evaluated on 100 equally-spaced points.
}
	\label{fig:pdf_comparison}
\end{figure}



\begin{figure}[!b]
	\centering
%	\subfigure[MISC, iteration 14]{\includegraphics[width=0.24\textwidth]{Fig_MISC/MISC_Contour_iter13_50by50.png}}
%	\subfigure[MISC, final iteration]{\includegraphics[width=0.24\textwidth]{Fig_MISC/MISC_Contour_iter30_50by50.png}}
%          \subfigure[SRBF, iteration 8]{\includegraphics[width=0.24\textwidth]{Fig_RBF/Contour-Iter0033.png}}
%	\subfigure[SRBF, final iteration]{\includegraphics[width=0.24\textwidth]{Fig_RBF/Contour-Iter0053.png}}
	\subfigure[MISC, iteration 14]{\includegraphics[width=0.45\textwidth]{Fig_MISC/MISC_Surface_iter13_50by50.png}}
	\subfigure[MISC, final iteration]{\includegraphics[width=0.45\textwidth]{Fig_MISC/MISC_Surface_iter30_50by50.png}}
	\subfigure[SRBF, iteration 8]{\includegraphics[width=0.45\textwidth]{Fig_RBF/Surf-Iter0033.png}}
	\subfigure[SRBF, final iteration]{\includegraphics[width=0.45\textwidth]{Fig_RBF/Surf-Iter0053.png}}
	\caption{Comparison of MISC and SRBF results: response surfaces.}
	\label{fig:response_surface_comparison}
\end{figure}

\begin{figure}[!b]
	\centering
	\subfigure[MISC, iteration 14]{\includegraphics[width=0.45\textwidth]{Fig_MISC/points_iter13.png}}
	\subfigure[MISC, final iteration]{\includegraphics[width=0.45\textwidth]{Fig_MISC/points_iter30.png}}
           \subfigure[SRBF, iteration 8]{\includegraphics[width=0.45\textwidth]{Fig_RBF/TS_Iter33.png}}
	\subfigure[SRBF, final iteration]{\includegraphics[width=0.45\textwidth]{Fig_RBF/TS_Iter53.png}}
	\caption{Comparison of MISC and SRBF results: points in parameter space. Note that every point required on grid $\mathcal{M}_i$ is required also on all the grids with lower refinement level.}
	\label{fig:points_comparison}
\end{figure}


\begin{figure}[!b]
	\centering
	\subfigure[MISC, cumulative number of simulations]{\includegraphics[width=0.45\textwidth]{Fig_MISC/total_points.png}}
	\subfigure[MISC, number of new simulations]{\includegraphics[width=0.45\textwidth]{Fig_MISC/new_points.png}}
           \subfigure[SRBF, cumulative number of simulations]{\includegraphics[width=0.45\textwidth]{Fig_RBF/TS_Size.png}}
           \subfigure[SRBF, number of new simulations]{\includegraphics[width=0.45\textwidth]{Fig_RBF/TS_Increase.png}}
	\caption{Comparison of MISC and SRBF results: number of simulations required at each iteration for each grid. }
	\label{fig:beta_points_comparison}
\end{figure}

% RISULTATI SRBF
\begin{figure}[!t]
	\centering
	\subfigure[]{\includegraphics[width=1\textwidth]{Fig_RBF/Umax-Conv.png}}
	\subfigure[]{\includegraphics[width=1\textwidth]{Fig_RBF/Umax-Conv_Det.png}}
	\caption{SRBF results: (a) convergence of the maximum prediction uncertainty and (b) its comparison with the lowest-fidelity prediction uncertainty and the normalized (with the function range) RMSE of $\mathcal{T}_1$ versus the computational cost from iteration $8$ to final.}
	\label{fig:points_RBF}
\end{figure}

\begin{figure}[!t]
	\centering
	\subfigure[MISC, iteration 14]{\includegraphics[width=0.45\textwidth]{Fig_MISC/indices_iter13.png}}
	\subfigure[MISC, final iteration]{\includegraphics[width=0.45\textwidth]{Fig_MISC/indices_iter30.png}}
	\caption{MISC results: explored multi-indices. The indices $\beta_1$ and $\beta_2$ determine how many quadrature points are selected according to the level function \eqref{eq:lev_fun} for the advancement speed and the draught, respectively.}
	\label{fig:indices_MISC}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=1\textwidth]{Fig_MISC/profits.png}
	\caption{MISC results: profit of the explored multi-indices at the final iteration. The multi-indices circled in yellow have profit higher than the one marked in red and have been added to the index set $\bm{I}$ (see Algorithm \ref{algo:misc_implementation}).}
	\label{fig:profits_MISC}
\end{figure}

Fig. \ref{fig:EV_comparison} shows the convergence of the expected value and standard deviation of $R_T$ versus the computational cost. MISC and SRBF converge towards similar estimates. MISC achieves good estimate already with low computational cost, whereas at later iterations, corresponding to computational cost above 1000, its behavior worsens; conversely SRBF gives a more stable estimate. Similar conclusions can be drawn by looking at the plot of the values of the standard deviation. Complementary information are given in Tab. \ref{table:comparison}, summarizing the expected value and the standard deviation achieved by the two methods at the final iteration and at one characteristic iteration. In the case of MISC iteration 14 (associated to a computational cost equals to 900) is selected, one of the iterations giving a good estimate of the expected value but before the ``disruption'' happening around cost approximately 1000. Such iteration is indicative of the behavior of MISC and the successive discussions are referred to it.
{Concerning SRBF, the} convergence of the expected value and the standard deviation is oscillatory (zoom not shown for brevity). The oscillation becomes more evident after iteration $8$ with computational cost of $4638$, {which is then selected as characteristic iteration for the SRBF and shown in Tab. \ref{table:comparison}). Actually,} after this iteration the SRBF moves from interpolation to {least-squares} approximation for the lowest fidelity only, since its number of training points reaches the threshold value of $5^N$. This produces oscillations in the last part of the SRBF convergence. Nevertheless, variations are small and oscillations limited.

Fig. \ref{fig:pdf_comparison} shows the $R_T$ histogram and {the estimate of the PDF of $R_T$ obtained using a kernel density estimation method}.
{Crucially, the values of $R_T$ used build histograms and the approximate PDF can be obtained cheaply, by evaluating the MISC and SRBF surrogate models over a suitable number of Monte Carlo samples from the parameter space.} 
The PDF obtained with SRBF has a peak around in the interval 20-40. A similar peak is retrieved also by MISC. However, in the latter case secondary peaks are observed for higher values of resistance at the final iteration. SRBF with exact interpolation (see Fig. \ref{fig:pdf_comparison}c) leads to a peak value significantly higher than MISC and SRBF with least-squares regression (see Fig. \ref{fig:pdf_comparison}a, b, and d).
{The spurious peaks in the PDF obtained with MISC can be explained by looking at the MISC response surface for $R_T$, which we discuss next.}

{The response surfaces obtained by the two methods} are shown and compared in Fig. \ref{fig:response_surface_comparison}. Once again, it can be observed that the behavior of MISC deteriorates at later iterations. The response surface is very irregular and this can be attributed to the numerical noise which affects the CFD simulations {(due to the fact that the solver implements an iterative method
  which stops as soon as a prescribed tolerance is met)}, in particular the one on the coarsest grid.
As the overall idea of MISC is to solve most PDEs on the less expensive grids and building the surrogate model with lagrangian (hence exact) interpolation, 
the presence of numerical noise turns out to be problematic for this method. This issue could be mitigated by doing e.g. a least-squares regression on the data, to smooth the numerical oscillations. A more thorough investigation of this aspect is out of scope here and will be considered in a future work (see also discussion in Sect. \ref{sect:conclusions} - Conclusions).
% One could also take advantage of the soft information (monotonicity, multimodality, ...) on the physical nature of the problem. In this particular case, the resistance is expected to be monotonically increasing with respect to advancement speed and draught. Such property could be preserved by employing, e.g., least-squares regressions with appropriate polynomial degree and/or monotonic smoothing \cite{dykstra1982}. Investigating this aspect is out of scope here and it will be considered in a future work.
On the contrary, SRBF suffers the numerical noise of the CFD outputs {only as long as} exact interpolation is imposed (see Fig. \ref{fig:response_surface_comparison}c) leading to a significant deformation of the response surface close to the lower bound of both the uncertain parameters,
whereas {for later iterations (i.e., larger computational costs)}
the use of regression improves the quality of the surrogates by smoothing the response surface
and filtering out the numerical noise (see Fig. \ref{fig:response_surface_comparison}d). 

Fig. \ref{fig:points_comparison} displays the points in the uncertain parameter space selected by MISC and SRBF. The two plots on the top line show the points employed by MISC at iteration 14 and at the final iteration. At the beginning the MISC algorithm explores more {the variability of the advancement speed}, suggesting a stronger dependence of the quantity of interest on {this parameter} rather than on the draught.
Points exploring {the variability of the draught} are added only at later iterations (this subject is elaborated also later on).
The sampling performed by SRBF is shown in Figs. \ref{fig:points_comparison}c and Figs. \ref{fig:points_comparison}d {at iteration 8} and {at the} final iteration, respectively. Until iteration $8$ (exact interpolation only), the adaptive sampling method explores the domain extrema and starts to cluster samples in two zones among $U=[7,8.8]$ m/s, since the numerical noise negatively affects the prediction uncertainty of the interpolating SRBF. Switching to the least-squares approximation and filtering out the noise prevents an excessive clusterization of the samples at the successive iterations. Indeed, the SRBF samples are fairly spread over the domain. 

Fig. \ref{fig:beta_points_comparison} shows the amount of simulations on the different spatial grids required by both methods at each iteration. Specifically, on the left the total number of simulations is displayed, whereas on the right only the number of new simulations asked at each iteration is shown. MISC required most of the simulations on the coarse grid; only five simulations on the finest grid are required (one at iteration 5, two at iteration 28, and two at iteration 30). 
At iteration 12, 24, and 25 no new points are added, which can be explained as follows. At iteration 12 the MISC algorithm requires simulations for spatial index $\alpha=5$: however, having considered only four spatial refinements level, this grid was not available. The profit of this multi-index is then set to zero and the algorithm restarts to explore from the multi-index with the next highest profit. 
Instead, at iteration 24 and 25 there is no new index $\jj$ to be added to the multi-index set because none of the indices $\jj \in \text{Mar}(\bm{I})$ would lead to $\bm{I} \cup \{\jj\}$ downward closed, see Algorithm \ref{algo:misc_implementation}. As for SRBF, it {spent} about 50\% of the final computational cost at the first iteration, then requiring simulations on the finest grids only at iterations 5 and 6. In all the other iterations mainly low-fidelity simulations are performed. This sampling behavior is due to the high values of prediction uncertainty that are found in the corners of the variables domain, because the topology of the initial training leads to extrapolation in those zones. 
%In that regions the highest prediction uncertainty is estimated and the adaptive sampling procedure have required all the fidelities, before moving to explore other regions.
Such corner regions are those with the highest estimated prediction uncertainty,
and the adaptive sampling procedure requires all the fidelities before moving
to explore other regions.


Fig. \ref{fig:points_RBF}a shows the maximum prediction uncertainty versus the computational cost. After the first four iterations the value of the maximum prediction uncertainty decreases from 120\% of the high-fidelity function range (R$_1$) to about 25\%. During the adaptive sampling the value of the maximum prediction uncertainty continues to decrease slower than in the first iterations, achieving a final value of about 5\%. The convergence shows some oscillations around a computational cost equal to 4600, due to the change from exact interpolation to least-squares approximation of the training set. 
%
Fig. \ref{fig:points_RBF}b compares the convergence of the maximum prediction uncertainty with its low-fidelity component and the normalized (with the function range) RMSE of the lowest-fidelity training set from iteration $8$. It is worth noting that the lowest-fidelity prediction uncertainty is almost equal to the maximum multi-fidelity prediction uncertainty until a computational cost of about 4655, thus representing its main component. %After lowest-fidelity samples are added, the lowest-fidelity components decrease significantly and a $\mathcal{M}_3$ simulation is requested. Therefore, the $U_{\hat{\varepsilon}_3}$ component of the prediction uncertainty is reduced and the low-fidelity metamodel prediction uncertainty component is again the greatest. Finally, the NRMSE of the fourth fidelity training set is almost constant and its value is significantly smaller than the maximum prediction uncertainty.

% RISULTATI MISC



Finally, coming back to the analysis of the MISC results, in Fig. \ref{fig:indices_MISC} the multi-indices $\left[\alpha, \beta_1,\beta_2\right]$ selected by the MISC method until iteration 14 and at the final iteration are shown. It can be seen that the multi-index set at iteration 14 stretches more in direction ``advancement speed''
{($\beta_1$)} than in direction ``draught'' {($\beta_2$)}:
this further confirms the statement already made that the parameter advancement speed is deemed more influential by MISC, i.e. the multi-indices with larger profits are predominantly found in direction advancement speed. More quantitative information on the profits can be found in Fig. \ref{fig:profits_MISC}, where the profit of every explored multi-index is displayed. Note that only the indices with the highest profits (marked in yellow) are added to the multi-index set $\bm{I}$. The remaining indices are explored (i.e. added to the multi-index set $\bm{G}$, therefore contribute to the MISC approximation) but non yet selected (i.e. added to the multi-index set $\bm{I}$). As already explained earlier on, there is no profit associated to the multi-index $\left[5,1,1\right]$ since the fifth spatial refinements level is not available.














